Algorithms for Markov Binomial Chains

We study algorithms to analyze a particular class of Markov population processes that is often used in epidemiology. More specifically, Markov binomial chains are the model that arises from stochastic time-discretizations of classical compartmental models. In this work we formalize this class of Markov population processes and focus on the problem of computing the expected time to termination in a given such model. Our theoretical contributions include proving that Markov binomial chains whose flow of individuals through compartments is acyclic almost surely terminate. We give a PSPACE algorithm for the problem of approximating the time to termination and a direct algorithm for the exact problem in the Blum-Shub-Smale model of computation. Finally, we provide a natural encoding of Markov binomial chains into a common input language for probabilistic model checkers. We implemented the latter encoding and present some initial empirical results showcasing what formal methods can do for practicing epidemiologists.

==> tables/ModestUltimate.tex <==
\begin{table}[]
    \centering
    \caption{Performance of Modest for large populations. Modest was run for the popinc properties in increasingle larger populations in a \emph{start of an epidemic} situation. We ran Modest with the max run lenght set to $0$ and seed $997$.}
    \begin{tabular}{|c|c|c|}
        \hline
         population & result &Modest simulation time \\
        \hline
     (10, 1, 1, 1) & 0.9961538461538462 & 6.1s  \\
     (20, 1, 1, 1) & 0.993 & 9.3s  \\
     (40, 1, 1, 1) & 0.993 & 11.7s  \\
     (80, 1, 1, 1) & 0.9971428571428571 & 12.1s  \\
     (160, 1, 1, 1) & 0.9936842105263158 & 25.2s  \\
     (320, 1, 1, 1) & 0.9983606557377049 & 27.7s  \\
     (640, 1, 1, 1) & 0.9952380952380953 & 68.1s  \\
     (1280, 1, 1, 1) & 1 & 74.7s  \\
     (2560, 1, 1, 1) & 0.9944444444444445 & 257.1s  \\
     (5120, 1, 1, 1) & 0.9944444444444445 & 504.0s  \\
     (10240, 1, 1, 1) & 0.9983606557377049 & 689.8s  \\
     (20480, 1, 1, 1) & 0.9952380952380953 & 1869.1s  \\
     (40960, 1, 1, 1) & 0.9983606557377049 & 2774.2s  \\
     (81920, 1, 1, 1) & 0.9971428571428571 & 6420.6s  \\
     (163840, 1, 1, 1) & 1 & 8882.6s  \\
     (327680, 1, 1, 1) & 0.9952380952380953 & 29609.8s  \\
     (0, 1, 1, 1) &  & s  \\
     (0, 1, 1, 1) &  & s  \\
     (0, 1, 1, 1) &  & s  \\
     (0, 1, 1, 1) &  & s  \\

         \hline
    \end{tabular}
    \label{tab:popincultimate}
\end{table}

==> tables/StormModestPrecision.tex <==
\begin{table}[]
    \centering
    \caption{The precision of Modest compared to the exact values in Storm. Note that for the EoE property, we used width 0.9 to keep the run time manageable in storm. The random number generator for Modest was set to 997.}
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        property & population & Storm & Modest (width 0.01) &   Modest (width 0.001)  \\
        \hline
         popinc&(3, 0, 0, 0) & 1 & 1 & 1 \\
         &(0, 1, 1, 1) & 0.9987240195 & 1 & 0.9989641434262948  \\
         &(3, 1, 1, 0) & 0.9952634065 & 0.9971428571428571 & 0.9955811462238886\\
         &(2, 1, 1, 1) & 0.9948733242 & 0.9971428571428571 & 0.9953703703703703\\
         &(1, 4, 0, 0) & 0.9972593727 & 0.9905982905982906  &  0.9971220260936301  \\
         \hline
         EoE &(3, 0, 0, 0) & 0 & 0 & 0 \\
         &(0, 1, 1, 1) & 275.6801531 & 276.65685600648203  & TO \\
         &(3, 1, 1, 0) & 285.2523967 & 285.1537294071891 & TO \\
         &(2, 1, 1, 1) & 348.3760444 & 348.7204048428036 & TO \\
         &(1, 4, 0, 0) & 255.5465313 & 255.65503788941862 & TO \\
         \hline
         OS &(3, 0, 0, 0) & 0 & TO & TO\\
         &(0, 1, 1, 1) & 1 & 1 & 1\\
         &(3, 1, 1, 0) & 0.999876224 & 1 & 1\\
         &(2, 1, 1, 1) & 0.9999997331 & 1 & 1 \\
         &(1, 4, 0, 0) & 1  & 1 & 1\\
         \hline
    \end{tabular}
    \label{tab:modestprecision}
\end{table}

==> tables/tableSIRStormParams.tex <==
\begin{table}[b]
    \centering
    \caption{Scalability of Storm on EoE property for SIR model.}
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        &&& dd-to-sparse & & dd-to-sparse\\
        population & sparse &  dd \& BuDDy & BuDDy &  dd \& Sylvan & Sylvan  \\
        \hline
        (5, 5, 0) & 0.074s & 402.931s   & 68.813s    & 14.552s    & 0.276s    \\
        (10, 10, 0)& 1.524s & 1682.572s  & 175.385s   & 312.827s   & 7.408s    \\
        (15, 15, 0)& 18.908s & 4446.139s  & 467.44s    & 1984.448s  & 61.682s   \\
        (20, 20, 0)& 118.889s & 15285.464s & 1796.469s  & 9194.601s  & 412.937s  \\
        (25, 25, 0)& 521.013s & MO         & 8483.432s  & 31162.389s & 2008.203s \\
        (30, 30, 0)& 1825.479s & MO         & 21577.803s & MO         & 7932.179s \\
        (35, 35, 0)& MO & MO         & MO         & MO         & MO        \\
        
        \hline
    \end{tabular}
    \label{tab:sirtractable}
\end{table}
